Simultaneously Learning Stochastic and Adversarial Bandits under the Position-Based Model

Online learning to rank (OLTR) interactively learns to choose lists of items from a large collection based on certain click models that describe users' click behaviors. Most recent works for this problem focus on the stochastic environment where the item attractiveness is assumed to be invariant during the learning process. In many real-world scenarios, however, the environment could be dynamic or even arbitrarily changing. This work studies the OLTR problem in both stochastic and adversarial environments under the position-based model (PBM). We propose a method based on the follow-the-regularized-leader (FTRL) framework with Tsallis entropy and develop a new self-bounding constraint especially designed for PBM. We prove the proposed algorithm simultaneously achieves $O(\log{T})$ regret in the stochastic environment and $O(m\sqrt{nT})$ regret in the adversarial environment, where $T$ is the number of rounds, $n$ is the number of items and $m$ is the number of positions. We also provide a lower bound of order $\Omega(m\sqrt{nT})$ for adversarial PBM, which matches our upper bound and improves over the state-of-the-art lower bound. The experiments show that our algorithm could simultaneously learn in both stochastic and adversarial environments and is competitive compared to existing methods that are designed for a single environment.

==> Algorithm_aaai.tex <==
\section{Algorithm}\label{sec:algo}

\begin{algorithm}[tb]
\caption{FTRL-PBM}
\label{alg:ftrlpbm}
\textbf{Input}: $\cX$.
\begin{algorithmic}[1]
\STATE $\hL_0=\mathbf{0}_{n\times m}$, $\eta_t=1/(2\sqrt{t})$. \label{algline1}
\FOR{$t=1,\dots,T$}
    \STATE Compute 
    \begin{align*}
        x_t=\argmin_{x\in\Conv(\cX)}\langle x, \hL_{t-1}\rangle + \frac{1}{\eta_t}\Psi(x)\,;
    \end{align*} \label{algline3}
    \STATE Sample $X_t\sim P(x_t)$; \label{algline4}
    \STATE Observe $\ell_{t,i,j}$ for those $(i,j)$-th entries satisfying $X_{t,i,j}=1$;
    \STATE Compute the loss estimator $\hat{\ell}_{t,i,j}=\frac{\ell_{t,i,j} \cdot \bOne{X_{t,i,j}=1}}{\xtij}$; \label{algline6}
    \STATE Compute $\hat{L}_t=\hat{L}_{t-1}+\hl_t$. \label{algline7}
\ENDFOR
\end{algorithmic}
\end{algorithm}

This section presents our main algorithm, $\ftrlpbm$, in Algorithm \ref{alg:ftrlpbm} for both stochastic and adversarial environments under PBM. Our $\ftrlpbm$ algorithm follows the general follow-the-regularized leader (FTRL) framework, whose main idea is to follow the action which minimizes the regularized cumulative loss of the past rounds. Since the complete loss vectors cannot be observed in the bandit setting, usually an unbiased estimator $\hat{\ell}_{t}$ satisfying $\EE{t}{\hat{\ell}_{t}}=\ell_t$ would serve as a surrogate.

Specifically, our algorithm $\ftrlpbm$ keeps track of the cumulative estimated loss $\hL_{t}=\sum^{t}_{s=1} \hat{\ell}_s \in \mathbb{R}_+^{n \times m}$ and initializes it as a zero vector (line \ref{algline1}). At each round $t$, $\ftrlpbm$ first computes a regularized leader $x_t$ in the convex hull of the action set $\Conv(\cX)$ by
\begin{align} 
    \label{eq:main}
    x_t=\argmin_{x\in\Conv(\cX)} \inner{x}{\hL_{t-1}} + \frac{1}{\eta_t}\Psi(x)
\end{align}
where $\Psi(x)$ is the regularizer (line \ref{algline3}). Here we take the $1/2$-Tsallis entropy
\begin{align*}
% \label{eq:regularizer}
    \Psi(x)= \sum_i-\sqrt{x_i} 
    % \label{eq:regularizer}
\end{align*}
as our regularizer, which is shown optimal for BOBW MAB \cite{zimmert2019optimal}. For BOBW semi-bandits, the optimal algorithm adopts a hybrid regularizer \cite{zimmert2019beating}, which may not be efficient for PBM and will be discussed later.

% Discussions about the challenges are put in Section \ref{sec:discussions}.

% It is also part of the hybrid regularizer adopted in the work for BOBW CMAB with semi-bandits \cite{zimmert2019beating}. It is not direct to prove the effectiveness of Tsallis entropy for PBM problem and we will discuss about its challenges in \shuai{xxx}.

Then $\ftrlpbm$ samples an action $X_t \sim P(x_t)$ from $\cX$ (line \ref{algline4}) where $P(x_t)$ satisfies $\EE{X\sim P(x_t)}{X}=x_t$. We follow previous works \cite{kale2010non,helmbold2009learning} to construct $P(x)$. The method is to first complete matrix $x_t$ into  a doubly stochastic matrix $M_t$, which is a convex combination of permutation matrices by Birkhoff's theorem, and then decompose matrix $M_t$ into its convex combination of at most $n^2$ permutation matrices by Algorithm 1 of \cite{helmbold2009learning}. The time complexity of whole sampling procedure is of order $O(n^{4.5})$ and the details can be found in Appendix \ref{app:opt}.

After observing the semi-bandit feedback for the selected action $X_t$, we can construct the unbiased estimator for the loss vector as
\begin{align*}
    \hat{\ell}_{t,i,j}=\frac{\ell_{t,i,j} \cdot \bOne{X_{t,i,j}=1}}{\xtij}
\end{align*}
for the $(i,j)$-th entry (line \ref{algline6}). Then the cumulative estimated loss $\hL$ is updated (line \ref{algline7}).


%Here $y_{t}=X_{t} \circ \ell_{t}$ represents the observed entries in the loss vectors. %\zhao{What does $\circ$ denotes? Is it the hardmard product? But $y_{t,i,j}$ seems not a matrix?}

\subsection{Optimization}  \label{sec:cbp}
% \zhao{
% There are two remaining issues in the implementation of Algorithm \ref{alg:ftrlpbm}:
% the constrained convex optimization problem (line 3 in Algorithm \ref{alg:ftrlpbm}) and the permutation matrix decomposition problem (line 4 of Algorithm \ref{alg:ftrlpbm}).
% The constrained convex optimization problem could be solved by the Frank-Wolfe algorithm \cite{frank1956algorithm}. 
% % In each iteration of Frank-Wolfe algorithm in our context, it computes an instance of the maximal matching in a bipartite graph166
% % in $O(n^{2.5})$ time using the Hopcroft–Karp algorithm \cite{hopcroft1973n}. The computation of $x_t$ ends in $O(n^{2.5}K)$
% % time where $K$ is the maximal iteration number of Frank-Wolfe algorithm. 
% % It is shown that the primal convergence rate of Frank-Wolfe algorithm satisfies $f(x^{(k)})-f(x^\ast)\leq O(\frac{1}{k})$ where $x^\ast$ is the optimal solution of $f(x)=\langle x, \hL_{t-1}\rangle+\eta_t^{-1}\Psi(x)$ and $x^{(k)}$ is the solution in the $k$-th iteration of Frank-Wolfe algorithm \cite{dunn1978conditional,jaggi2013revisiting}. 
% % \chen{the complexity of each iteration of FW?} 
% In each iteration of Frank-Wolfe algorithm in our context, it computes an instance of the maximal matching in a bipartite graph in $O(n^{2.5})$ time using the Hopcroft–Karp algorithm \cite{hopcroft1973n}.
% The computation of $x_t$ ends in $O(n^{2.5}K)$ time where $K$ is the maximal iteration number of Frank-Wolfe algorithm.
% The solution of permutation matrix decomposition problem is discussed in \cite{kale2010non,helmbold2009learning}. The computation of the permutation matrix decomposition is efficient and it can be showed that the solution could be found in $O(n^{4.5})$ time.
% Please refer to Appendix \ref{app:opt} for the pseudo-code of the algorithms for the two core optimization problems and the complete discussions.
% }


%Since projecting onto the constrain set $\Conv(\cX)$ is rather expensive and the Tsallis entropy is not a gradient Lipschiz function, traditional convex optimization methods will be inefficient to solve problem (\ref{eq:main}).
It remains to solve the optimization problem Eq.\eqref{eq:main}. Let $f(x) = \langle x, \vone\rangle +\Psi(x)$. Then Eq.\eqref{eq:main} is equivalent to the following problem
\begin{align*}
    x_t=\argmin_{x\in\Conv(\cX)}\langle x, \hL_{t-1}\rangle + \frac{1}{\eta_t}f(x)\,.
\end{align*}
Since $f(x)$ is a Legendre function and $\Conv(\cX)$ is compact, the above equation can be solved by the following two-step procedure (see Chapter 28 of \cite{lattimore2020bandit})
\begin{align}
    \tilde{x}_t &=\argmin\ \langle x, \hL_{t-1}\rangle + \eta_t^{-1}f(x)\,, \label{eq:twostep1}\\
    x_t &=\argmin_{x\in\Conv(\cX)} D_f(x,\tilde{x}_t)\,, \label{eq:twostep2}
\end{align}
where $D_f$ denotes the Bregman divergence induced by the Legendre function $f$. Since $\hL_{t-1}$ is non-negative, we can guarantee that the minimum of Eq.\eqref{eq:twostep1} exists. Note that the linear term in $f(x)$ is necessary because $\langle x, \hL_{t-1}\rangle + \frac{1}{\eta_t}\Psi(x)$ does not have a minimum for the unconstrained case when any element of $\hL_{t-1}$ is equal to zero.

However, solving Eq.\eqref{eq:twostep2} is still not easy. Our idea is to leverage the cyclic Bregman projection (CBP) \cite{bregman1967the,bauschke2000dykstras}. We first decompose $\Conv(\cX)$ into two sets on which Bregman projection can be efficiently computed. Note that \cite{dunn1978conditional,mendelsohn1958the}
% \begin{align*}
%     \Conv(\cX)=\set{X\in[0,1]^{n\times m}~\Bigg|~\sum_{i=1}^n X_{i,j}=1, \forall j\in[m];~ \sum_{j=1}^m X_{i,j}\leq 1, \forall i\in[n]}\,.
% \end{align*}
\begin{align*}
    \Conv(\cX)=\left\{X\in[0,1]^{n\times m}~\Bigg|~\sum_{i=1}^n X_{i,j}=1, \forall j\in[m];\right.\\
    \left.\sum_{j=1}^m X_{i,j}\leq 1, \forall i\in[n]\right\}\,.
\end{align*}
Thus there is
$\Conv(\cX)=\cX_1\cap \cX_2$ where 
\begin{align*}
    &\cX_1=\set{X\in[0,1]^{n\times m}~\Bigg|~\sum_{i=1}^n X_{i,j}=1, \forall j\in[m]}\,,\\
    &\cX_2=\set{X\in[0,1]^{n\times m}~\Bigg|~ \sum_{j=1}^m X_{i,j}\leq 1, \forall i\in[n]}\,.
\end{align*}

Then we can solve Eq.\eqref{eq:twostep2} by the CBP algorithm presented in Algorithm \ref{alg:cbp}. The Bregman projection onto $\cX_1$ can be computed efficiently. Since the constraint in $\cX_1$ is column-wise, we can compute the projection of each column separately. For each column $j$, we need to solve
\begin{align*} %\label{eq:bpx1}
    \argmin_{\substack{\sum_{i=1}^n x_{i,j}=1\\ x_{i,j}\in[0,1]}} -\sum_{i=1}^n\sqrt{x_{i,j}}+\langle \vone-\nabla f(\tilde{x}_t)_j,x_j\rangle
\end{align*}
where $\nabla f(\tilde{x}_t)_j$ is the $j$-th column of $\nabla f(\tilde{x}_t)$. Similar to the implementation of \cite{zimmert2019optimal}, its solution %of Eq.\eqref{eq:bpx1} 
takes the form 
\begin{align} \label{eq:sol_x1}
   x_{i,j}=\frac{1}{4}(\nabla f(\tilde{x}_t)_{i,j}-\lambda-1)^{-2}
\end{align}
where $\lambda$ can be solved by 
\begin{align} \label{eq:sollam}
    \sum_{i=1}^n \frac{1}{4}(\nabla f(\tilde{x}_t)_{i,j}-\lambda-1)^{-2}=1\,.
\end{align}
This can be figured out approximately using Newton's method with only a few iterations. The Bregman projection onto $\cX_2$ is similar and all details are postponed to Appendix \ref{app:opt}.

\begin{algorithm}[t]
\caption{Cyclic Bregman Projection} \label{alg:cbp}
\begin{algorithmic}[1]
\STATE $x^0 =\tilde{x}_t$, $s=0$.\\
\WHILE{not converge}
    \STATE $s=s+1$\\
    \STATE $x^{2s-1} = \argmin_{x\in\cX_1} D_f(x,x^{2s-2})$\\
    \STATE $x^{2s} = \argmin_{x\in\cX_2} D_f(x,x^{2s-1})$\\
\ENDWHILE
\end{algorithmic}
\end{algorithm}

\begin{remark}
Note that the hybrid regularizer adopted in \cite{zimmert2019beating} may not be efficiently solved with low computational complexity by traditional convex optimization methods under PBM. 
The reason is that the computation of the projection onto the constrained set $\Conv(\cX)$ is rather expensive and the gradient of the hybrid regularizer is not Lipschitz continuous. The Tsallis entropy works since we can get a closed form of Eq.\eqref{eq:sol_x1}. It is an open question whether the FTRL with the hybrid regularizer can be solved efficiently under PBM.
\end{remark}
% Note that our optimization method could be inefficient if the algorithm adopts the hybrid regularizer as in \cite{zimmert2019beating}. The main issue is that we cannot get a closed form as Eq.\eqref{eq:sol_x1} for the hybrid regularizer

% \paragraph{Constrained Convex Optimization} Line 3 in Algorithm \ref{alg:ftrlpbm} is a canonical constrained convex
% optimization problem. Note that the minimizer of Eq.\eqref{eq:main} is constrained in the convex hull of $\cX$. To avoid computing the projection for the feasible domain, we consider the well-known Frank-Wolfe (FW) \cite{frank1956algorithm} algorithm (\emph{a.k.a.},  conditional gradient method) due to its projection-free property. Let $K$ be the maximal iteration number in Algorithm \ref{alg:regLeader}. It starts at an initial point $x^{(0)}=x_{t-1}$. At the $k$-th iteration, Algorithm \ref{alg:regLeader} first computes the gradient of $f(\cdot)=\langle \cdot,\hL_{t-1} \rangle+\eta_t^{-1}\Psi(\cdot)$ at $x^{(k)}$. To compute $s^{(k)}$, it moves towards to boundary of the convex hull $\Conv(\cX)$ along the negative gradient direction. Note that the objective function of computation of $s^{(k)}$ is linear and could be solved efficiently using the well-established linear programming methods. Then Algorithm \ref{alg:regLeader} will terminate if the threshold $\epsilon$ is satisfied and will continue to the next iteration otherwise. \chen{put the details of FW algorithm in the appendix.}

% \paragraph{Permutation Matrix Decomposition}
% Line 4 of Algorithm \ref{alg:ftrlpbm} could be viewed as a permutation matrix decomposition problem. To sample $X_t\sim P(x_t)$, we need to find a group of $n\times m$ permutation matrices whose convex combination is $x_t$. Actually, it can be shown that such a decomposition of any $x\in \Conv(\cX)$ exists and we could find the decomposition of $x$ in polynomial time. Follow  \citet{kale2010non}, we first change $x_t$ into a doubly stochastic matrix $W\in \BR^{n\times n}$, namely, each element $W_{i,j}\geq 0$ and $\sum^n_{j=1}W_{i,j}=\sum^n_{j=1}W_{j,i}=1$ for any $i\in [n]$, in $\cO(n^2)$ times (Line \ref{alg:decomposition:l1} in Algorithm \ref{alg:decomposition}). \citet{helmbold2009learning} show that a doubly stochastic matrix $W$ can be decomposed into the convex combination of at most $n^2-2n+2$ permutation matrices meaning that there are most $\cO(n^2)$ iterations on Line \ref{alg3:line2} of Algorithm \ref{alg:decomposition}. At each iteration, it needs to find a permutation matrix $\Pi^k$ such that $W_{i,\Pi^k(i)}>0$ for any $i\in [n]$. This is actually the problem of maximal matching in a bipartite graph and could be solved by the Hopcroft–Karp algorithm \cite{hopcroft1973n} at a cost of $\cO(n^{2.5})$ times. It follows that Algorithm \ref{alg:decomposition}
%  will end in $\cO(n^{4.5})$ times. \chen{put alg 3 in the appendix}

% This section briefly gives discussions on the two core optimization problems of $\ftrlpbm$, namely, the constrained convex optimization problem (Line 3 in Algorithm \ref{alg:ftrlpbm}) and the permutation matrix decomposition problem (Line 4 of Algorithm \ref{alg:ftrlpbm}). 
% \zhao{



% There are two remaining issues in the implementation of Algorithm \ref{alg:ftrlpbm}:
% the constrained convex optimization problem (Line 3 in Algorithm \ref{alg:ftrlpbm}) and the permutation matrix decomposition problem (Line 4 of Algorithm \ref{alg:ftrlpbm}).
% % }
% The constrained convex optimization problem could be solved by the Frank-Wolfe algorithm \cite{frank1956algorithm}. 
% It is shown that the primal convergence rate of Frank-Wolfe algorithm satisfies $f(x^{(k)})-f(x^\ast)\leq \cO(\frac{1}{k})$ where $x^\ast$ is the optimal solution of $f(x)=\langle x, \hL_{t-1}\rangle+\eta_t^{-1}\Psi(x)$ and $x^{(k)}$ is the solution in the $k$-th iteration of Frank-Wolfe algorithm \cite{dunn1978conditional,jaggi2013revisiting}. 
%\chen{the complexity of each iteration of FW?} 
% \zhao{
% In each iteration of Frank-Wolfe algorithm in our context, it computes an instance of the maximal matching in a bipartite graph in $\cO(n^{2.5})$ time using the Hopcroft–Karp algorithm \cite{hopcroft1973n}.
% The computation of $x_t$ ends in $\cO(n^{2.5}K)$ time where $K$ is the maximal iteration number of Frank-Wolfe algorithm.
% % } 
% The solution of permutation matrix decomposition problem is discussed in \cite{kale2010non,helmbold2009learning}. The computation of the permutation matrix decomposition is efficient and it can be showed that the solution could be found in $\cO(n^{4.5})$ time.
% % \zhao{
% % The pseudo-code of the algorithms for the two core optimization problems and the complete discussions are provided in Appendix \ref{app:opt}. 
% Please refer to Appendix \ref{app:opt} for the pseudo-code of the algorithms for the two core optimization problems and the complete discussions.
% }


 


% Let $\cD=[0,1]^{n\times m}\subset \BR^{n\times m}$.
% We define $\Psi_t(\cdot)=\eta_t^{-1}\Psi(\cdot)$ and $\Phi_t(\cdot)=\max_{x\in\Conv(\cX)}\langle x,\cdot \rangle-\Psi_t(x)$, which is the convex conjugate of $\Psi_t+\cI_{\Conv(\cX)}$. Thus we have

% \begin{eqnarray*}
% \Psi_t(x) &=& \sum_i -\frac{1}{\eta_t}\sqrt{x_i}\,,\\
% \nabla\Psi_t(x) &=& \sum_i-\frac{1}{2\eta_t}x_i^{-\frac{1}{2}}\,.
% \end{eqnarray*}
% For $y\leq 0$, we have
% \begin{align*}
%     \Psi_t^*(y) = \max_{x\in \cD}\langle x,y \rangle-\Psi_t(x)=\sum_i -\frac{1}{4\eta_t^2y_i}\,.
% \end{align*}
